A Case for Synthesis of Recursive Quantum Unitary Programs

Quantum programs are notoriously difficult to code and verify due to unintuitive quantum knowledge associated with quantum programming. Automated tools relieving the tedium and errors associated with low-level quantum details would hence be highly desirable. In this paper, we initiate the study of program synthesis for quantum unitary programs that recursively define a family of unitary circuits for different input sizes, which are widely used in existing quantum programming languages. Specifically, we present QSynth, the first quantum program synthesis framework, including a new inductive quantum programming language, its specification, a sound logic for reasoning, and an encoding of the reasoning procedure into SMT instances. By leveraging existing SMT solvers, QSynth successfully synthesizes ten quantum unitary programs including quantum adder circuits, quantum eigenvalue inversion circuits and Quantum Fourier Transformation, which can be readily transpiled to executable programs on major quantum platforms, e.g., Q#, IBM Qiskit, and AWS Braket.

==> Makefile <==
PAPER = main
TEX = $(wildcard *.tex)
BIB = references.bib
FIGS = $(wildcard figs/*.pdf figs/*.png graphs/*.pdf graphs/*.png)

.PHONY: all clean open o
all: $(PAPER).pdf

paper : $(PAPER).pdf

%.pdf: %.tex $(BIB) $(FIGS)
	pdflatex $(basename $@)
	bibtex $(basename $@)
	pdflatex $(basename $@)
	pdflatex $(basename $@)

open o: $(PAPER).pdf
	which open >/dev/null 2>/dev/null && open $< || \
	which xdg-open >/dev/null 2>/dev/null && xdg-open $<

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf

==> acknowledge.tex <==
%% Acknowledgments
\begin{acks}                            %% acks environment is optional
                                        %% contents suppressed with 'anonymous'
  %% Commands \grantsponsor{<sponsorID>}{<name>}{<url>} and
  %% \grantnum[<url>]{<sponsorID>}{<number>} should be used to
  %% acknowledge financial support and will be used by metadata
  %% extraction tools.
  This material is based upon work supported by the
  \grantsponsor{GS100000001}{National Science
    Foundation}{http://dx.doi.org/10.13039/100000001} under Grant
  No.~\grantnum{GS100000001}{nnnnnnn} and Grant
  No.~\grantnum{GS100000001}{mmmmmmm}.  Any opinions, findings, and
  conclusions or recommendations expressed in this material are those
  of the author and do not necessarily reflect the views of the
  National Science Foundation.
\end{acks}

==> chapter/cases/wstate.tex <==
\subsection{$2^n$-qubtis W-state Circuit}
\paragraph{Motivation}
To demonstrate our synthesizer's ability, we use it to do the contest problem "generate W-state" which appeared in Microsoft Q\# Coding Contest. The problem is: given $N = 2^n$ qubits in zero state $\ket{0^{\otimes N}}$, our task is to create a $N$-qubit W-state on them.
$N$-qubit W state is an equal superposition of all basis states on N qubits that have Hamming weight equal to 1:
\begin{align}
    \ket{W_N} = \frac{1}{\sqrt{N}}(\ket{100...0}+\ket{010...0} + ... + \ket{00...01})
\end{align}
For example, for $N=1, \ket{W_1} = \ket{1}$ and for $N=2, \ket{W_2} = \frac{1}{\sqrt{2}}(\ket{01}+ \ket{10})$. W-state is remarkable for representing a specific type of multipartite entanglement and for occurring in several applications in quantum information theory such as quantum teleportation\cite{shi2002teleportation} and quantum secure direct communication\cite{hai2006quantum}. In ensemble-based quantum memories\cite{fleischhauer2002quantum} area, W state's robustness against particle loss is a very beneficial property ensuring good storage properties.\par
\paragraph{Synthesis Process}
\name fails to generate a $N$-qubit W-state program without using any ancilla qubits. So we allow the \name to use qubit 0 as an ancilla qubit and synthesize a program $S$ that $S(n)$ generate a $2^n$-qubit W state on qubits $1\sim 2^n$ while keep qubit 0 in state $\ket{0}$. The specification is given by
\begin{align}
    h(n,x,y): \{x=0\},\qquad     \alpha(n,x,y)&:= \frac{1}{\sqrt{2^n}}\cdot\bvalue{((y-1)\&y)=0 \land y>1}
    \label{equ:wspec}
\end{align}
The hypothesis suggest the initial state is $\ket{0}^{\otimes N}$. From the definition of W state we know that for the output ket $\ket{y}$ whose hamming weight is one, its amplitude is 1. Otherwise its amplitude is 0. So $\alpha$ is given by
Here "\&" is bitwise \textbf{And} operation. The term $(y-1)\&y$ equals to 0 only if the hamming weight of $y$ is 1 or 0. So this term restrict $y$ be $\ket{0}$ or the state in the W-state. Since we need to keep qubit 0 in state $\ket{0}$, the combining term $y>1$ ensures $y$ is our target state. \name still fails to synthesize a W-state program in simple fixpoint structure with one ancilla. So we let \name synthesize in two steps.\par

In the first step, we let \name synthesize a program $S'$ given the specification $(h,\alpha)$
\begin{align}
    &h'(n,x,y): \{n>0\}\\
    &\alpha'(n,x,y):=\frac{1}{\sqrt{1}}\cdot \dvexp{\bvalue{y[0]=x[0]\oplus (\oplus y[2n:n+1]) \land ((x[0]=0 \land \mask(x,0)=\mask(y,0))\nonumber\\ 
    &\qquad \qquad \lor (x[0]=1 \land x[n:1]=y[2n:n+1] \land x[2n:n+1]=y[n:1]))
    }}{0}
\end{align}
Then \name generates a program $S'$ below
\begin{align*}
    S'&:= \fix_1~w~(\const{I})~(\const{cswap 0 1 n})~(\const{CNOT n 0})\\    w&:=(\shift{1}{n-1}{1})\cdot (\shift{n}{2n-2}{2})
\end{align*}


Then we use $S'$ as a known program and let \name try to synthesize a program based on the specification in Equation~\ref{equ:wspec}. This time \name successfully synthesizes  a program $S_w$ below, which generate a $2^n$-bit W-state
\begin{align*}
    S_w:= \fix_1~Id~(\const{X 1})~(\const{H 0})~(\const{S' $2^n$})
\end{align*}





==> chapter/goal.tex <==
\section{Synthesis Goal and Key Idea}
Our synthesis goal is: \textcolor{blue}{given $(h,\alpha)$ which can represent a unitary function $\U: \ujudge{h}{\U}{\alpha}$, find a program $P: \mathbb{Z}^+ \rightarrow \text{Unitary}$ that for all $n\in \mathbb{Z}^+$, $P(n)$ is same unitary as $\U(n)$.}\par The synthesis procedure can be divided into two steps:
\begin{enumerate}
    \item Search: enumerate all possible candidate program based on the program syntax.
    \item Verification: for each candidate program, try to verify that it is the desired program automatically. If succeed, return this program as result. If fail, move on to the next candidate program.
\end{enumerate}
The verification step is hard since we need to verify the equivalence between a unitary function $\U$ and a recursive program $P$. Each unitary function is exactly a function from $n$ to a $2^n\times 2^n$ matrix, so the problem is as hard as checking the equivalence between two matrix family automatically.\par
The \textcolor{red}{\textbf{key}} idea of our verification method: check the equivalence between $\U$ and $P$ inductively. An informal explanation of our idea: if we can

\begin{itemize}
\item For some constant base $b\in Z^+$, verify that $\forall n:0<n\le b, \U(n)=P(n)$.
\item Suppose for some $k$, we have $\forall n:0<n\le k-1, \U(n)=P(n)$, verify that $U(k)=P(k)$
\end{itemize}
Then we can say that for all $n\in \mathbb{Z}^+$, $P(n)$ is same unitary as the one $\U(n)$.\par
For example, when we meet the correct GHZ program $P$ during the search
\begin{figure}[h]
    \centering
    \begin{minipage}[m]{0.4\textwidth}
    \begin{coq}
Fixpoint GHZ n :=
    match n with
    | 1 => H 0
    | _ => GHZ n-1;  CNOT n-2 n-1
    end.
\end{coq}
    \end{minipage}
\begin{minipage}[m]{0.48\textwidth}
\centerline{

\Qcircuit @C=1.0em @R=1.0em {
& & \text{GHZ n-1}\\
&&&&&&&\\
    \lstick{\ket{0}} & \gate{H} & \ctrl{1} & \qw & \qw & \qw & \qw &\qw\\
    \lstick{\ket{0}} & \qw & \targ & \ctrl{1} & \qw & \qw & \qw &\qw\\
    \lstick{\ket{0} } & \qw & \qw & \targ &\qw & \qw & \qw & \qw & \rstick{\frac{\ket{0}^{\otimes n}+\ket{1}^{\otimes n}}{\sqrt{2}}}\\
       & \vdots & &&\ddots & & & \\
    \lstick{\ket{0}} &\qw& \qw & \qw & \qw & \targ & \ctrl{1} & \qw  \gategroup{2}{1}{7}{6}{0.7em}{--}\\
    \lstick{\ket{0}} &\qw & \qw &\qw & \qw & \qw & \targ & \qw \gategroup{3}{8}{8}{8}{1.2em}{\}}\\
}
}
\end{minipage}
\caption{Generation of the $n$-qubit GHZ state using quantum logic gates.}
\label{fig:ghz}
\end{figure}
We need to verify that for all $n$, it returns the same unitary as the unitary function represented by 
\begin{align}
    h_{GHZ}(n,x)&:= x==\ket{0}^n\\
    \alpha_{GHZ}(n,x,y)&:=\frac{\delta(y,\ket{0}^n) + \delta(y,\ket{1}^n)}{\sqrt{2}}
\end{align}
We first verify that when $n=1$, $P$ returns the unitary $H~0$ and it is our desired unitary. Suppose $H~0$ can be represented by a function $\alpha_H$, this verification step can be done by checking
$$
\forall x,y\in\{0,1\}^1, h_{GHZ}(1,x)\rightarrow \alpha_{GHZ}(1,x,y)=\alpha_H(1,x,y)
$$
Then for $n>1$, we suppose \texttt{GHZ }$n'$ give us the desired $2^{n'}\times 2^{n'}$ unitary and we just need to verify that appending a $\texttt{CNOT}~n-2~n-1$ will give us the desired $2^{n}\times 2^{n}$. Suppose $\texttt{CNOT}~n-2~n-1$ is a unitary function that can be represented by $\alpha_{CNOT}$, this verification step can be done by checking
\begin{align}
    \forall n'>1, \alpha_{GHZ}(n',x,y) = \texttt{seq}(\alpha_{GHZ}(n'-1, x',y'), \alpha_{CNOT}(n,x,y))
\end{align}
where 
\begin{align}
        \texttt{seq}(\alpha,\alpha') &= \lnxy  \sum_{z\in \{0,1\}^{n}} \alpha(n,x,z)\alpha'(n,z,y)\\
\end{align}
and $x',y'$ are the bit vectors that discard the highest bit in $x,y$.\par
This method simplify the problem from verifying the equivalence between two unitary function to verifying the equivalence between certain unitary and verifying the recursive feature of the given unitary function $\U$.\par
The following parts are the details about how to encode the verification part into an SMT solver.

==> chapter/justification.tex <==
\section{Unitary Function}
To synthesize an unitary for arbitrary dimension,
the expected program $\U$ is a function of unitary $$\U:\mathbb{Z}^+\rightarrow \text{Unitary}$$ For easy notation, $\U(n)$ returns a unitary applied on $n$ qubits $q_0,...,q_{n-1}$.
Automatically verifying a program satisfying the specification or not is an essential part of the synthesis.
 To implement automated verification for fixed size quantum circuits, \cite{amy2018towards} has developed a concrete representation of quantum operators as \textit{path-sums}.(Adavantage of path-sums here).\par We modify path-sum\cite{amy2018towards} to implement the automated verification for symbolic quantum circuits. 
\subsection{Original Path-sum}
\cite{amy2018towards}
\begin{definition}[path-sum]\label{def:sop}
	An $n$-qubit \textit{path-sum} $\xi$ consists of
	\begin{itemize}
		\item an \textit{input signature} $\ket{\x=x_1x_2\cdots x_n}$  where each $x_i$ is a (distinct) variable or Boolean constant,
		\item a \textit{phase polynomial} $P\in\D_M[\x,\y]$ over input variables $\x$ and \textit{path variables} $\y=y_1y_2\dots y_m$, and
		\item an \textit{output signature} $\ket{f(\x,\y)=f_1(\x,\y)\cdots f_n(\x,\y)}$ where each $f_i\in\F[\x,\y]$ is a Boolean polynomial.
	\end{itemize}
	The \textit{associated operator} of a path-sum is the partial linear map $U_{\xi}$ where
	\[
		U_{\xi} : \ket{\x} \mapsto \frac{1}{\sqrt{2^m}}\sum_{\y\in\F^m} e^{2\pi i P(\x,\y)}\ket{f(\x,\y)}.
	\]
\end{definition}
where  $\D=\{\frac{a}{2^b} | a, b \in \Z\}$ is the ring of \textit{dyadic fractions}, which correspond uniquely to multi-linear polynomials in $\D_M[\x]=\D[\x]/\langle x_i^2 - x_i\rangle$.
\subsection{Our Modification}
There are three shortages in the program verification with the original definition of path-sum:
\begin{itemize}
    \item The original definition of path-sum $\xi$ can only represent a fixed-size unitary and a fixed number of paths in the unitary. One path-sum can only mean a specified unitary, not a unitary family.
    \item An $m$-qubit unitary represented by $U_{\xi}$ is a map from all input signature in $\{0,1\}^m$. But in the application, we sometimes only focus on some of the legal inputs (i.e., for state preparation the inputs are usually $\ket{0}^m$), and it is redundant to verify the program satisfies the specification for all inputs.
    \item \cite{amy2018towards} verifies whether a given circuit $C$ has the same semantic with a path-sum $\xi$ by introducing a system of reduction rules for path-sums. The key feature of their calculus is that the reduction rules strictly decrease the number of path variables, producing a (not necessarily unique) normal form in polynomial time. This method works when the circuit has a fixed number of path variables. However, this limits their framework in that it can only verify one fixed size circuit in one verification procedure. It cannot verify a circuit family in which the circuit's size is symbolically parameterized.
\end{itemize}
So we define our representation for unitary function as below:

Under some precondition $h$, each unitary function $\U$ can be represented by a function $ \alpha_U: \mathbb{N}\times \{0,1\}^{n} \times \{0,1\}^{n}\rightarrow \mathbb{C}$ where
    \begin{itemize}
        \item $n\in \mathbb{N}$ denotes that $U$ is unitary on qubits $q_0,...,q_{n-1}$.
        \item $x,y \in \{0,1\}^{n}$ are two $n$ length bit vector denoting the input signature and path variables.
    \end{itemize}
The relation between $\alpha_{\mathcal{U}},h$ and the unitary function $\U$ is restricted by:
\begin{align}
    \forall n\in \mathbb{N}, \forall x,y\in \{0,1\}^{n} \nonumber\\  
    h(n,x)\rightarrow \U(n) \ket{x}=\sum_y \alpha_\U(n, x, y)\ket{y}
\end{align}
and we say
\begin{align}
    \ujudge{h}{\U}{\alpha_U}
\end{align}
Given an arbitrary $2^n\times 2^n$ unitary matrix $M$, we can set $h_M(n,x)=\text{True}, \alpha_M(n,x,y) = M_{xy}$ and then $M$ can be represented by $h_M, \alpha_M$. So our representation can represent arbitrary unitary.\par
Compare with the original definition of path-sum\cite{amy2018towards},
\begin{itemize}
    \item The amplitude function for each path is parameterized by $n$, not only $x,y$.
    \item We restrict the number of path variables to $2^n$(all possible paths) and represent the amplitude of each path with a function $\alpha$, whose value can be 0 to remove the redundant path, rather than $e^{2\pi i P(\x,\y)}$. In this way, the exact number of paths is decided by the value of the amplitude function $\alpha$. We can utilize an SMT solver to symbolically check the equivalence between two unitary functions $\xi,\zeta$ under the same precondition easily by checking the equivalence between two functions $\alpha_{\xi}, \alpha_{\zeta}$.
    \item  Since our representation has included all possible paths, we restrict the output signature equals to path variables $\ket{y}$ which will make the verification easier while not limits the expressiveness.
    \item The precondition $h$ allows the user to express some preconditions for the input state $x$ and the unitary size $n$. For example, for the state preparation program, the input state is usually $\ket{0}^n$; for the $n'$-bit adder circuit, it always has an even size ($2n'$).
\end{itemize}

==> chapter/oracle.tex <==
\section{Synthesize Quantum Programs with Oracle}

We extend \name to Oracle-\name for synthesizing quantum programs with oracles (e.g. the Deutsch-Jozsa algorithm~\cite{deutsch1992rapid}). 
The new synthesis is more challenging because: 
(1) one needs to specify the property of the oracle as part of the synthesis specification (e.g., the oracle for Deutsch-Joza algorithm is constant or balanced); (2) the verification of generated programs satisfying specifications should hold for any legal oracle. 
The second one is in particular hard since it involves formulas containing a function variable bounded by a quantifier $\forall$, which is not directly supported by any SMT solver. % or other automatic verification tools. 

We address the first challenge by defining a new specification, \emph{oracle specification}, which allows users to express the oracle's properties. 
Unfortunately, we do not have a general solution to the second challenge. 
However, for interesting cases, we identify a work-around which enables us to synthesize the program for the Deutsch-Jozsa problem~\cite{deutsch1992rapid}.

%In the following section, we explain the definition of \emph{oracle specification} and how to encode the oracle function into SMT solver. Then we discuss how to extend \name to Oracle-\name and use Oracle-\name to solve  as an example.


\subsection{Oracle Specification} \label{sec:oracle_spec}
To synthesize a quantum algorithm with an $n$-bit oracle function $f:\{0,1\}^n \rightarrow \{0,1\}^m$, users need to give an \emph{Oracle Specification} instead of the hypothesis-amplitude specification. 
Typical quantum algorithms deal with promised problems, where promised conditions are assumed for the oracle, and should behavior accordingly when different promises hold. 
To model that, 
%The oracle used by a quantum algorithm sometimes has one of many properties, and the users expect the program to give different results based on the oracle's property. Some 
\emph{Oracle Specification} is defined as a set of tuples $\{(p^f, h, \alpha)_i\}$ where $(h,\alpha)$ is the hypothesis-amplitude specification and $p^f$ is a precondition that describes the promised condition of the oracle $f$. %, describing $f$'s property. 
Namely, for program $S^f$ with oracle instantiated by $f$, we have,
\begin{align} \label{eq:oracle_spec}
    p^f \rightarrow \interpret{h}{S^f}{\alpha}~.
\end{align}
The size of the oracle specification set is simply the number of different promises. 
The new synthesizer Oracle-\name will try to generate \sqirs programs that satisfy (\ref{eq:oracle_spec}) for all tuples in the specification set.
% An oracle specification suggests Oracle-\name try to generate a ISQIR program $S^f$ that satisfies different hypothesis-amplitude specification $(h,\alpha)$ under different precondition $p^f$. 
% That is, for each $(p^f, h, \alpha)$ tuple in the given oracle specification, we have
% \begin{align}
%     p^f \rightarrow \interpret{h}{S^f}{\alpha}~.
% \end{align}
Let us study a concrete example as follows. 
%We show the oracle specification for the $n$-bit Deutsch-Jozsa algorithm as an example. 

The oracle used by the $n$-bit Deutsch-Jozsa algorithm is a function $\{0,1\}^n\rightarrow \{0,1\}$. The oracle is either \emph{constant} or \emph{balanced} so that there are two promises in the specification: 
\begin{align}
    p^f_1:~\sum_{j\in \{0,1\}^n} f(j) = 2^{n} \lor \sum_{j=0}^{2^n-1} f(j) = 0, \qquad
    p^f_2:~\sum_{j\in \{0,1\}^n} f(j) = 2^{n-1}.
\end{align}
When the oracle $f$ is constant,  either $\forall j, f(j)=1$ or $\forall j, f(j)=0$. The first case suggests $\sum_{j\in \{0,1\}^n} f(j) = 2^{n}$ and the second suggests $\sum_{j\in \{0,1\}^n} f(j) = 0$. 
Thus, $p^f_1$ implies that $f$ is constant. 
In the balanced case, we have $\sum_{j\in \{0,1\}^n} f(j) = 2^{n-1}$ which is implied by $p^f_2$.

To synthesize an $n$-bit Deutsch-Jozsa program, it suffices to synthesize a unitary $U$ which, when applied to the initial state, can help  
distinguish the two promises of the oracle. 
Suppose we start from the initial state $\ket{0}^{n+1}$ and measure the result state in the computational basis. 
We could desire the output is always $\ket{1}\ket{0}^n$ if the oracle is constant, and is any orthogonal state if the oracle is balanced. Precisely, such specification for $(h_1, \alpha_1), (h_2, \alpha_2)$ could be intuitively given by 
%We want the measurement result to always be $\ket{1}\ket{0}^n$ if the oracle is constant and yield another state if the oracle is balanced. So we can give the specification for $(h_1, \alpha_1), (h_2, \alpha_2)$ as 
\begin{align}
    h_1&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n \land n>0\},\qquad \alpha_1(n,x,y)=\pm 1,\\
    h_2&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n \land n>0\},\qquad \alpha_2(n,x,y)=0.
\end{align}
%($h_1,\alpha_1$) suggests $(\alpha(n+1,\ket{0}^{n+1}, \ket{1}\ket{0}^{n}))^2$, the property of yielding state $\ket{1}\ket{0}^{n}$, is 1 when the oracle $f$ is constant (implied by $p^f_1$); ($h_2, \alpha_2$) suggests the property of yielding state $\ket{1}\ket{0}^{n}$ is 0  when the oracle $f$ is balanced (implied by $p^f_2$).

\subsection{Extend \name to Oracle-\name}
The overall workflow of Oracle-\name is similar to \name's workflow shown in Fig~\ref{fig:overview} except for the following differences:
\begin{itemize}[leftmargin=2mm]
    \item The specification from the user is changed from a hypothesis-amplitude specification $(h,\alpha)$ to an oracle specification $\{(p^f, h, \alpha)_i\}$.
    \item We extend ISQIR's syntax and the ISQIR logic to allow one more  rule for calling the oracle in the program. The new syntax and its corresponding rule are
    \begin{align*}
        S::= \cdots \mid \oracle{O_f} \qquad   \qquad \qquad             \inferrule*[Right=Oracle]{ \alpha\equiv^{{\mathbb N}^3}\lambda n.\sem{O_f}}{\mathbb{N}^3\triangleright (\oracle{O_f})\leftrightarrow\alpha}
    \end{align*}
    where $O_f$ refers to a \sqir implementation of the oracle $f:\{0,1\}^n\rightarrow \{0,1\}^m$ and its semantics refers to a unitary that maps $\ket{x}\ket{y} \mapsto \ket{x}\ket{y\oplus f(x)}, x\in \{0,1\}^n, y\in \{0,1\}^m$. 
    %Oracle-\name syntax-guided searcher is based on this new syntax and each candidate program $S_O$ generated by the searcher is a map from an oracle function to a ISQIR program.
    \item Oracle-\name's verifier is also different from \name's verifier. Given a candidate program $S_c$ and an oracle specification, Oracle-\name's verifier tries to verify that for each $(p^f,h,\alpha)$ tuple in the specification, whether we have $\interpret{h}{S_c}{\alpha}$ under precondition $p^f$.
    If the answer is "Yes" for all tuples, $S_c$ is sent to the backend compiler and the synthesis terminates. Otherwise, the synthesizer continues with a new program candidate. 
    %a new candidate program will be required from the Oracle-\name Searcher.
\end{itemize}

\subsection{Encoding the Oracle and the Deutsch-Jozsa Example}
The second challenge of synthesizing a quantum algorithm with oracle is how to encode an oracle function into the SMT solver. For a function $f:\{0,1\}^n\rightarrow \{0,1\}^m$, one could concatenate all its value $f(0)f(1)...f(2^n-1)$ together and get a ($2^n\cdot m$)-bit vector $V$, which could be encoded into SMT instances. 
However, the length of the bit vector will unfortunately depend on the input and output domain size of the function $f$, which cannot be used as SMT encodings if one wants to synthesize \sqirs programs that work for an arbitrary input size. 
We feel that this limitation likely holds for general oracles and any work-around should leverage the special properties of oracles in any given problem. 

Indeed, in the following, we showcase how the specific promises of the oracle in the Deutsch-Jozsa problem can help use circumvent the aforementioned difficulty in synthesis.  

%This approach equips a function with 
%In this way, one one-to-one map a $\{0,1\}^n\rightarrow \{0,1\}^m$ function to a $2^n\cdot m$-bit vector. Since a bit vector can be one-to-one mapped to the binary representation of an integer, a $\{0,1\}^m\rightarrow \{0,1\}^n$ oracle function can be mapped to an integer and be encoded into the SMT solver.
% For example, Oracle-\name verifier needs to verify the formula below during the verification step of the synthesis for $n$-bit Deutsch Jozsa program.
% \begin{align}
%         \forall f:\{0,1\}^n\rightarrow \{0,1\},~ \forall i\in \{0,1\}^n, ~ 2\cdot f(i) - 1 = \bvalue{f(i)\neq 0}-\bvalue{f(i)=0}.
% \end{align}
% With the encoding method for the oracle function $f$, Oracle-\name encode this formula as an SMT instance
% \begin{align}
%     \forall N_f \in \nat,~ \forall
%      i \in [0,2^n-1], ~ 2\cdot N_f[i]=\bvalue{N_f[i]\neq 0}-\bvalue{N_f[i]= 0}.
% \end{align}

%We let Oracle-\name try to synthesize a program for the Deutsch Jozsa problem as an example.
%Consider a Deutsch Jozsa problem:

% Precisely, Given a function $f:\{0,1\}^n \rightarrow \{0,1\}$. The given function $f$ has the promise that it is one of these two types:
% \begin{enumerate}
%     \item $f$ is a constant function (i.e. 0 on all inputs or 1 on all inputs)
%     \item $f$ is a balanced function (i.e. ($f$ returns 1 for half of the input domain and 0 for the other half).
% \end{enumerate}
% The problem is to synthesize a quantum program that can distinguish $f$'s type.

% Given a function $f:\{0,1\}^n \rightarrow \{0,1\}$. Let $I_0$ be the input bit-strings of length $n$ where the first bit is 0 and $I_1$ be the remaining ones (i.e. the first bit is 1). The given function $f$ has the promise that it is one of these two types:
% \begin{enumerate}
%     \item The total number of strings in $I_0$ for which $f(x)=0$ plus the total number of strings in $I_1$ for which $f(x)=1$ is $2^{n-1}$.
%     \item $f(x)=0$ for all $x\in I_0$ and $f(x)=1$ for all $x\in I_1$.
% \end{enumerate}
% The problem is to synthesize a quantum program that can distinguish $f$'s type.

Recall the oracle specification given in Section~\ref{sec:oracle_spec}: 
\begin{align}
    p^f_1&:~\sum_{j\in \{0,1\}^n} f(j) = 2^{n} \lor \sum_{j=0}^{2^n-1} f(j) = 0, \qquad
    p^f_2:~\sum_{j\in \{0,1\}^n} f(j) = 2^{n-1}.\\
        h_1&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n\land n>0\},\qquad \alpha_1(n,x,y)= \pm 1,\\
    h_2&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n\land n>0\},\qquad \alpha_2(n,x,y)=0.
\end{align}
% \begin{align}
%     p^f_1&:~ \sum_{i\in \{0,1\}^n} i[0]\cdot f(i) + (1-i[0])\cdot(1-f(i))= 2^{n-1}, \\ 
%     h_1&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n\},\qquad \alpha_1(n,x,y)=0 ,\\
%     p^f_2&:~ \sum_{i\in \{0,1\}^n} i[0]\cdot f(i) + (1-i[0])\cdot(1-f(i))= 2^{n},   \\  
%     h_2&:~\{x=\ket{0}^{n+1} \land y=\ket{1}\ket{0}^n\},\qquad \alpha_2(n,x,y)= 1.
% \end{align}
Let us demonstrate how to verify the specification of the
candidate program $S$:
\begin{align}
    S&:=\const{X 0};\const{H 0};~S_H;~ \oracle{O_f};~ S_H;\\
    \text{where } S_H &:= \fix_1~Id~(\const{I})~(\const{I})~(\const{H n}).
\end{align}
Note that $S_H$ is an \sqirs program applying Hardmard gates on qubits $q_1\sim q_n$. Note that the \sqirs program $S$ is the textbook version of the Deustch-Jozsa quantum algorithm for any input size $n$. 
To verify $S$ against the oracle specification, one needs to establish:
\begin{align}
    p^f_1\rightarrow (\interpret{h_1}{S}{\alpha_1}),\qquad
    p^f_2\rightarrow (\interpret{h_2}{S}{\alpha_2}).
\end{align}
Oracle-\name first uses the \textsc{CONST} rule to extract the $(h,\alpha)$ triple of each \textbf{const} component in $S$ and uses the \textsc{FIX} rule to build the $(h,\alpha)$ triple for program $S_H$. Then it uses the new \textsc{ORACLE} rule to prove that $\interpret{\nat^3}{\oracle{O_f}}{\alpha_f}$ and 
\begin{align}
    &\alpha_f(n,x,y) := \bvalue{x[n+1:1]=y[n+1:1] \land y[0]=f(x[n:1])\oplus x[0]}, 
\end{align}
which suggests that $\oracle{O_f}$ maps state $\ket{q_0} \ket{q_1q_2...q_n}$ to state $\ket{q_0 \oplus f(q_1q_2...q_n)} \ket{q_1q_2...q_n}$. 
Then Oracle-\name uses the \textsc{SEQ} rule, the \textsc{WEAKEN} rule and the \textsc{REPLACE} rule several times to sequence these components together, which eventually leads to 
% \begin{align}
%     &\interpret{h_1}{S}{\alpha_P},~\interpret{h_2}{S}{\alpha_P},\\
%     &\alpha_P(n,x,y):= \frac{1}{2^{n-1}}\sum_{i\in \{0,1\}^n} (1-2\cdot f(i))\cdot (1-2\cdot i[0]).
% \end{align}
\begin{align}
    &\interpret{h_1}{S}{\alpha_P},~\interpret{h_2}{S}{\alpha_P},\\
    &\alpha_P(n,x,y):= \frac{1}{2^{n-1}}\sum_{i\in \{0,1\}^n} \bvalue{f(i)=1}-\bvalue{f(i)=0}.
\end{align}

It is important to observe that both preconditions $p^f_1$, $p^f_2$ and the amplitude function $\alpha_P(n,x,y)$ only involve the sum of oracle function values over all possible inputs. 
This special feature removes the need to treat individual outputs of function $f$, i.e., $f(0), f(1), \cdots, f(2^n-1)$ separately. 
Instead, one only needs to keep track of their sum and proves something that uniformly holds for all inputs, which can be handled by existing SMT solvers. 
First, Oracle-\name tries to utilize the SMT solver to search two integer $a,b$ that satisfy
\begin{align}
    \forall f~\forall i\in {0,1}^n~, \bvalue{f(i)=1}-\bvalue{f(i)=0} = a\cdot f(i)+b.
\end{align}
This is achieved by replacing the term $f(i)$ with a $\{0,1\}$-valued variable and solving the following new formula with variable $a, b$ by the SMT solver:
\begin{align}
    \forall z\in \{0,1\}~, \bvalue{z=1}-\bvalue{z=0} = a\cdot z+b.
\end{align}
whose solution is $a=2$ and $b=-1$. Hence we have
\begin{align}
        \forall f~\forall i\in \{0,1\}^n~, \bvalue{f(i)=1}-\bvalue{f(i)=0} = 2\cdot f(i)-1,
\end{align}
which connects $\alpha_P(n,x,y)$ with the sum of function values by 
\begin{align}
    \alpha_P(n,x,y)= \frac{1}{2^{n-1}}\sum_{i\in \{0,1\}^n} (\bvalue{f(i)=1}-\bvalue{f(i)=0}) = \frac{1}{2^{n-1}}\sum_{i\in \{0,1\}^n} (2\cdot f(i)-1).
\end{align}

Henceforth, Oracle-\name can verify that 
\begin{align}
 &\sum_{i\in \{0,1\}^n} f(j) = 2^{n-1} \rightarrow \alpha_P(n,x,y)=0,\\
 &\sum_{j\in \{0,1\}^n} f(j) = 2^{n} \lor \sum_{j=0}^{2^n-1} f(j) = 0 \rightarrow \alpha_P(n,x,y) = \pm 1,
\end{align}
which implies 
\begin{align}
    p^f_1 \rightarrow \alpha_P \equiv^h \alpha_1,\qquad p^f_2 \rightarrow \alpha_P \equiv^h \alpha_2.
\end{align}
By the \textsc{REPLACE} rule,  $S$ is shown to satisfy the given oracle specification
\begin{align}
    p^f_1\rightarrow (\interpret{h_1}{S}{\alpha_1}),\qquad
    p^f_2\rightarrow (\interpret{h_2}{S}{\alpha_2}).
\end{align}
%We explain the idea that $S$ can solve this variant Deutsch Jozsa problem in Appendix~\ref{sec:explain}.

%\input{chapter/backup/oracle}



==> chapter/representation.tex <==
\section{Hypothesis-amplitude Representation}
Saurabh \etc\cite{srivastava2010program}'s program synthesis framework shows the benefits of interpreting program synthesis as generalized automated program verification. We follow the same insight in our framework: we define a \emph{\logicName} representation for quantum operators and automate the quantum program verification based on this representation. Inspired by recent work on quantum program verification\cite{amy2018towards,qbricks2020deductive}, we design our \logicName representation based on Richard Feynman’s \textit{path integral} technique, which has also been used to prove results in complexity theory\cite{dawson2004quantum,montanaro2017quantum}, to perform circuit simulation\cite{koh2017computing,bravyi2016improved} and optimization\cite{amy2018controlled,amy2014polynomial,amy2019tcount}. The idea of Feynman's \textit{path integral formulation} is to describe the amplitude of a quantum state by an integral over all possible paths leading to that state. In practice, as a quantum circuit is usually modelled as an operator on a Hilbert space, a discrete sum-over-paths technique rather than integral is typically used \cite{bacon2008analyzing,dawson2005solovay,montanaro2017quantum,koh2017computing,amy2018towards,amy2018controlled,amy2014polynomial,amy2019tcount,koh2017computing,bravyi2016improved,qbricks2020deductive}. We can describe a sum-over-paths abstractly as a discrete set of paths $T\in \mathbb{Z}_2^m$, together with an \textit{amplitude}
function $\psi$ and state transformation $f$ representing the operator
\begin{align*}
    U:\ket{x} \mapsto \sum_{y\in T} \psi(x,y) \ket{f(x,y)}
\end{align*}
All representations based on the sum-over-paths technique in these previous works\cite{amy2018towards,qbricks2020deductive,bacon2008analyzing,dawson2005solovay,montanaro2017quantum,koh2017computing,amy2018towards} share in common that the amplitude $\psi(x,y)$ of all possible paths have the same \textit{magnitude} and only the \textit{phase}s of the amplitude are different between paths. These forms of the same \textit{magnitude} but different \textit{phase} are so typical in many quantum algorithms so that they can be used as a succinct representation in the verification of many quantum algorithms, which makes it useful for synthesis purposes.\par
One limitation of this sum-over-paths technique is that it only addressed fixed-size quantum operators and cannot be used for the verification of \sqirs programs directly. So we expand the previous amplitude function $\psi(x,y)$ to a new amplitude function $\alpha(n,x,y)$ which can be parametrized by an entry index $n$. During the synthesis for a quantum program, we sometimes have a hypothesis for the initial quantum state (i.e. the initial state is usually $\ket{0}^\otimes n$ for state preparation program). So we also define a hypothesis set to express this knowledge.
% In our framework, for a \sqirs program $S$ and an amplitude function $\alpha$, when we have $\interpret{\nat^3}{S}{\alpha}$, $S(n)$ can be viewed as a partial linear map by the Definition~\ref{def:judge}
% \begin{align}
%     S(n): \ket{x}\mapsto \sum_{y\in \nat} \alpha(n,x,y) \ket{y}
% \end{align}
% It can also be written in a equivalent form
% \begin{align*}
%     S(n): \ket{x}\mapsto \sum_{y: \alpha(n,x,y)\neq0} \alpha(n,x,y) \ket{y}  
% \end{align*}
% In this form, we can find that
% $S(n)$ is an operator that can also be represented by a sum-over-paths in which the transformation function $f$ is identity and the set of paths $T$ is $\{y | \alpha(n,x,y)\neq 0\}$. We design our amplitude function $\alpha$ based on sum-over-paths with this intuition.

% \subsection{Encoding syntax of \logicName}
% For the hypothesis set $h$, we restrict $h$ in the form
\begin{definition}[Hypothesis Set]
 A hypothesis set $h$ is defined as
 \begin{align}
    h:\{(n,x,y) \mid B(n,x,y) \}
\end{align}
where $B(n,x,y)$ is a \textit{Boolean} expression constructed by the variables $n,x,y$. The hypothesis in this form suggests we only focus on the entries $(n,x,y)$ that makes the Boolean expression $B(n,x,y)$ true.
\end{definition}
% , and $S^1$ is the unit circle of complex plane:
% \begin{align*}
%     \alpha(n, x, y)=(p, \beta) \Leftrightarrow U_P(n, x, y)=\frac{p}{\sqrt{2}^\beta}.
% \end{align*}
% Here $U_P$ is the unitary of program $\F$'s semantics. Although this representation is not complete for every possible unitary programs, it covers many applications.
 We restrict the amplitude function $\alpha$ in the below form that all possible paths have the same magnitude but different phase
\begin{definition}[Amplitude Function]
An amplitude function $\alpha$ is in the form
 \begin{align}
    \alpha(n,x,y)&:= \frac{1}{\sqrt{\beta(n)}} \dvexp{\bvalue{B(n,x,y)}}{V(n,x,y)}
    %\\S(n)&:\ket{x}\mapsto \frac{1}{\sqrt{2}^{\gamma(n)}} \sum_{y\in \mathbb{N}} \sum_{i=0}^m \delta_i(n,x,y) \cdot e^{2\pi i P_i(n,x,y)} \ket{y}    
\end{align}
where 
\begin{itemize}
    \item $\beta$ is a natural number expression constructed only by $n$ and it decides the magnitude of all possible paths.
    \item $B$ is a boolean expression constructed by $(n,x,y)$. $\bvalue{B}:\text{Bool}\rightarrow \{0,1\}$ is a function that returns 1 if $B$ is True and returns 0 otherwise. 
    %, satisfying $\forall n~x~y\in \mathbb{N}, \sum_{i=0}^k \bvalue{B_i(n,x,y)}\le 1$;
    \item $V$ is a natural number expression constructed by $(n,x,y)$ and it decides the phase of each path's amplitude.
    \item   For $x\in \mathbb{N}$, suppose $x$'s binary representation is $x_q...x_1x_0$ where $x_i\in \{0,1\}$, we use $d(x)$ to denote the fractional binary notation of $x$
    \begin{align}
    d(x) = [0.x_0x_1...x_q] = \sum_{i=0}^q x_i \cdot 2^{-(i+1)}
\end{align}  
\end{itemize}
\end{definition}
 Fig.~\ref{fig:halpha} shows the syntax we allow to construct the expressions $\beta, B, V$. All these syntax are supported by the SMT solver. For the expression $\beta$, since we focus on the state in which all possible paths' amplitudes have the same magnitude, $\beta$ only depends on $n$ and does not depend on $x,y$. For the boolean expression $B$, since function $\alpha$ has non-zero value \textit{iff} $B(n,x,y)$ is true, $B$ exactly decides the path set $T$ as $\{y | B(n,x,y)\}$. \par
By restricting $\alpha$ in this form, we disassembled the complex number function $\alpha$ into the combination of three integer or boolean expressions. Thus we can represent this complex number function $\alpha$ with a set of SMT expressions which enable us to encode the calculation in Definition~\ref{def:calculation} into the SMT solver. This will be discussed in Section~\ref{sec:encode-cal} %Restricting $\alpha$ in this form does not reduce its expressiveness, and $\alpha$ still suffices to express the specification for generating the most interesting unitary. 
% % In specific, it can cover all quantum operations that can be represented by the original path-sums.
% \begin{theorem}
% Given a $n'$-qubit Mat Amy's path-sum $\xi$ and its corresponding unitary $U_\xi$ is in the form:
% 	\[
% 		U_{\xi} : \ket{\x} \mapsto \frac{1}{\sqrt{2^m}}\sum_{\y\in\mathbb{Z}^m} e^{2\pi i P(\x,\y)}\ket{f(\x,\y)}.
% 	\]
% There exists a \logicName $h-\alpha$ satisfies that when a \sqirs program $S$ has $\interpret{h}{S}{\alpha}$, $\sem{\ssem{S}(n')}$ is the same unitary as $U_\xi$
% \end{theorem}
% \begin{proof}
% \textcolor{red}{Theorem does not hold since the original path-sum can cover some strange cases}
% \end{proof}
% For a Boolean vector $\u\in \Z^{k}$, we use $B(\u)$ to denote the $k$-bit natural number whose binary representation is $\u$. Since $P$ is a dyadic fractions polynomial and $f$ is a Boolean polynomial over $\Z^{n'}$, there exists two functions $V_P, V_f:\nat^3\rightarrow \nat$ generated by our syntax that has
% \begin{align*}
%     &\forall \x \in \Z^{n'}~\y \in \Z^{m},\\ P(\x,\y) = d(V_P(n', B(\x), B(\y)))\\
%     B(f(\x,\y)) = V_f(n', B(\x), B(\y))
% \end{align*}
% Let a \logicName as 
% \begin{align*}
%     h&:= \{(n,x,y)| n=n'\land x<2^{n'} \land y<2^{n'}\\
%     \alpha&:= \frac{1}{\sqrt{2}^{m}} \sum_{i=0}^m \dvexp{\bvalue{y=V_f(n,x,i)}}{V_P(n,x,i)}
% \end{align*}

==> chapter/syntax.tex <==

\section{Unitary Function}
%\newcommand{\U}{\mathcal{U}}
Our synthesis target program is a unitary function that can produce desired unitary for arbitrary dimension, not some constant size unitary. 
The expected result program $\U$ is a function of unitary 
$$
\U:\mathbb{Z}^+\rightarrow \text{Unitary}
$$
For easy notation, $\U(n)$ returns a unitary applied on $n$ qubits $q_0,...,q_{n-1}$.\par
Under some hypothesis $h$, each unitary function $\U$ can be represented by a complex number function $ \alpha_U: \mathbb{N}\times \{0,1\}^{n} \times \{0,1\}^{n}\rightarrow \mathbb{C}$ where
    \begin{itemize}
        \item $n\in \mathbb{N}$ denotes that $U$ is unitary on qubits $q_0,...,q_{n-1}$.
        \item $x,y \in \{0,1\}^{n}$ are two $n$ length bit vector denoting the input signature and path variables.
    \end{itemize}
The relation between $\alpha_\U,h$ and the unitary function $\mathcal{U}$ is restricted by:
\begin{align}
    \forall n\in \mathbb{N}, \forall x,y\in \{0,1\}^{n} \nonumber\\  
    h(n,x,y)\rightarrow \U(n) \ket{x}=\sum_y \alpha_\U(n, x, y)\ket{y}
\end{align}
and we say
\begin{align}
    \ujudge{h}{\U}{\alpha_U}
\end{align}
For example, $n$-qubit QFT circuit
\begin{align*}
    \text{QFT:} \ket{x} \mapsto \frac{1}{\sqrt{2^n}} \sum_{y=0}^{2^n-1} e^{\frac{2\pi i\cdot xy}{2^n}} \ket{y}
\end{align*}
So
\begin{align}
    h(n,x,y)&:=\text{\textbf{True}} \\
    \alpha_{QFT}(n,x,y) &:=  \frac{1}{\sqrt{2^n}} e^{\frac{2\pi i\cdot xy}{2^n}}
\end{align}
% For the $n$-qubit GHZ circuit
% \begin{align*}
%     \ket{GHZ}_n : \ket{0}^n \mapsto \frac{\ket{0}^{\otimes n} + \ket{1}^{\otimes n}}{\sqrt{2}}
% \end{align*}

\section{Expression Language for Unitary Function}
\label{sec:express}
We use a function $\alpha(n, x, y)$ to represent a unitary function, where $n$ is a natural number, $x, y$ are strings in $\{0, 1\}^n$
% , and $S^1$ is the unit circle of complex plane:
% \begin{align*}
%     \alpha(n, x, y)=(p, \beta) \Leftrightarrow U_P(n, x, y)=\frac{p}{\sqrt{2}^\beta}.
% \end{align*}
% Here $U_P$ is the unitary of program $\F$'s semantics. Although this representation is not complete for every possible unitary programs, it covers many applications.

To encode it into SMT instance, we further restrict $(h,\alpha)$ by the syntax shown in Fig.~\ref{fig:halpha}. The value of $p$ to be in the \textit{binary expression representation} form $\sum_j \delta_j e^{-2\pi i d(v_j)}$, where $\delta_j$ is an $\{0, 1\}$-valued function taking in $n, x, y$, $v_j$ is a bit vector function taking in $n, x, y$, and $d(l)=0.l_{1}l_{2}...$ is a real number in $[0, 1)$ for a bit-vector $l$.\par 
\begin{figure}[h]
    \centering
    \begin{tabular}{ccc}
      $m\in\mathbb{Z}$ & $n\in \mathbb{N}$ Number of qubits in $\alpha_U$  & $x,y:$ BitVector 
    \end{tabular}
\begin{align*}
    \text{Spec} &::=\quad (h, \alpha)\\
    \text{Hypothesis }h&::=\quad \lnxy ~b\\
    \text{U Function }\alpha &::=\quad \lnxy ~ \frac{1}{\sqrt{2}^\beta}\cdot p\\
    \text{Amplitude }p & ::=\quad p_1 + p_2 \mid \dvexp{\delta}{v}\\
    \text{Delta }\delta&::= \delta_1\cdot \delta_2 \mid \tif(b, 1, 0)\\
    \text{BoolExp }b & ::=\quad \text{\textbf{True}} \mid \text{\textbf{False}} \mid b_1 \land b_2 \mid b_1 \lor b_2 \\
    &\quad\mid v_1==v_2 \mid v_1<v_2 \mid v_1>v_2 \\
    \text{BitVecExp }v & ::=\quad x \mid y \mid n \mid \texttt{bv}(m) \mid v[v'] \mid v[v_1:v_2] \\
    &\quad \mid v_1+v_2 \mid v_1*v_2 \mid r(v) \\
    \text{Exponent }\beta &::=\lambda n. \quad m \mid n \mid n+m \mid m*n
\end{align*}   
\caption{Syntax of the
specification $h, \alpha_U$ and the calculation rule. In the expression $\dvexp{b}{v}$, the boolean expression $b$ is evaluated as 1 if it is true else 0. Each unitary funtion $G$ in database is also represented by an U function $\alpha_G$. $\texttt{bv}(m)$ means to transfer an $n$-bit signed integer $m$ into an corresponding $n$-bit bitvector. $r(v)$ means to reverse the order of bits in $v$}
\label{fig:halpha}
\end{figure}
% \textcolor{blue}{Given specified $\x,\y$, the amplitude of path $\y$ in the original path-sum is represented by $e^{2\pi i P(\x,\y)}$, which is a unit vector in the complex plane.  
% In our representation, this amplitude is represented by $\sum_j \delta_j e^{-2\pi i d(v_j)}$. So we add restriction $\forall n,x,y, \sum_j \delta_j\leq 1$ for our representation so that the summation degenerates to one term when given a specified $n,x,y$, without reducing our representation's expressiveness compared with the original path-sums. Since SMT solver does not support trigonometric calculation, this additional restriction enables us to check the equivalence between two-phase $p_1,p_2$ with SMT solver.}\par

With a hypothesis set $H=\{h(n, x,y)~:~\forall n, x, y\}$, the SMT encoding of checking equivalence of $\alpha_1, \alpha_2$ encoded as
\begin{align*}
    \alpha_1=\lnxy \frac{1}{\sqrt{2}^\beta}\sum_j \delta_j e^{-2\pi i d(v_j)}\\
    \alpha_2=\lnxy \frac{1}{\sqrt{2}^{\beta'}}\sum_j \delta_j' e^{-2\pi i d(v'_j)}
\end{align*}
 reduces to
\begin{align*}
    &\forall n, x, y, ~~ h(n, x, y)\rightarrow\\ &\begin{cases}\beta(n)=\beta'(n) \\ \sum_j \delta_j(n, x, y)=\sum_j \delta_j'(n, x, y) \\
    \sum_j \delta_j(n, x, y) \le 1 \land \sum_j \delta_j'(n, x, y)\le 1\\
    \sum_j \delta_j(n, x, y) v_j(n, x, y)=\sum_j \delta_j'(n, x, y) v_j'(n, x, y)\end{cases}.
\end{align*}
and we say
\begin{align}
    \ufeq{h}{\alpha_1}{\alpha_2}
\end{align}
%  Then we consider the concatenation of two programs in representations $\alpha_1$ and $\alpha_2$, where we need to calculate:
% \begin{align*}
%     \texttt{seq}(\alpha_1,\alpha_2)=\lnxy \uplus_{z\in\{0, 1\}^n} \alpha_1(n, x, z)\utimes \alpha_2(n, z, y),
% \end{align*}
% where $\uplus$ and $\utimes$ is defined over $\mathbb{C} \times \nat$ by 
% \begin{align*}
%     (p_1, \beta)\uplus(p_2, \beta)&=(p_1+p_2, \beta), \\
%     (p_1, \beta_1)\utimes(p_2, \beta_2)&=(p_1 p_2, \beta_1+\beta_2).
% \end{align*}

\subsection{Sequence of $\alpha$}
In the sequence rule of the unitary function, we need to calculate 
\begin{align*}
    \texttt{seq}(\alpha_1,\alpha_2)=\lnxy \sum_{z\in\{0, 1\}^n} \alpha_1(n, x, z) \alpha_2(n, z, y),
\end{align*}
This cannot be done efficiently since there are $2^n$ terms. The composition rule in \cite{amy2018towards} does not meet this problem since they just need to consider fixed number terms. This problem is as hard as symbolic size matrix multiplication and is hence non-trivial in general. In application, we can calculate this term efficiently only when one of $\alpha_1$ or $\alpha_2$ is sparse. We say a function $\alpha$ is sparse if: there exists two constant-size sets $M^x, M^y$ and their elements are some functions $n \times \{0,1\}^n \rightarrow \{0,1\}^n$ and satisfy
\begin{align}
    &\forall n, \forall x,y\in\{0,1\}^{n},\quad \alpha(n,x,y)\neq 0 \leftrightarrow \nonumber\\
    &(\exists! p\in M^x, p(n,y) = x) \land (\exists! q\in M^y, q(n,x) = y)
\end{align}
This means that: given specified $y,n$, $\alpha$ is a function of $x$ denoted as $f^x_\alpha$. Then $f^x_\alpha$ should be a function that has non-zero value on only $O(1)$ points. Similar to the function $f^y_\alpha$.
Suppose $\alpha_2$ is sparse and the corresponding sets are $M^x$, then the sum can be transformed to
\begin{align}
    \sum_{z\in \{0,1\}^{n}} \alpha_1(n,x,z)\alpha_2(n,z,y) = \sum_{t\in M^x,z=t(n,y)} \alpha_1(n,y,z) \alpha_2(n,z,y)
    \label{equ:inductcheck}
\end{align}
This sum expression on the right hand has only $O(1)$ terms so we can calculate it efficiently.\par
% \subsection{Constant-size program}
% The program syntax for constant-size program is similar to a unitary \emph{SQIR} program. A unitary program$U$ is a sequence of applications of gates G to qubits q.
% \begin{align*}
%     U::=U_1;U_2\mid G~q\mid G~q_1~q_2 
% \end{align*}
% Qubits are referred to by natural numbers that index into a global register of quantum bits. Each program is parameterized by a set of unitary one- and two-qubit gates (from which G is drawn)
% and the dimension of the global register (i.e., the number of available qubits).\par
% \subsubsection{Encoding of constant-size program}
% Relation between $(h,\alpha)$ and $U$.
% \subsection{Parametrized Program syntax}
\section{Program Syntax}
The program constructed by our syntax is a unitary function $\F:\Z^+\rightarrow U$. Our syntax is

\begin{align*}
    &n: \text{Input of the unitary function,}\quad m\in \mathbb{Z}^+\\
    \F&::=I \mid G~0\mid G~0~1 \mid \texttt{Relabel}(\pi,\F')\\
    & \qquad\mid \F_1;\F_2 \mid \texttt{Fix}_k(\gamma(n),\F_0,\F_1,...,\F_{k-1},\F_l,\F_r) \mid O_f\\% \mid \text{Other successfully synthesized programs}\\
   %\G&::=  \mid  \\
    \pi&: \text{ A permutation over $(\mathbb{Z}_n,+)$}\\
    \pi&::= I \mid (0~u) \mid (1~u) \mid \sigma_m \mid \pi_1\pi_2\\
    u&::= m \mid n-m \mid n/m,~m\in \mathbb{Z}^+\\
        \gamma(n) &::= n-m\mid n/m\\
\end{align*}
Our program $\F$ is constructed by
\begin{itemize}
\item $I$ is the unitary function that always returns a $2^n\times 2^n$ unitary. $G~0$ returns a unitary that applies a known gate ($i.e. H,X,Y,Z$) on qubit $q_0$ and Identity gate on $q_1,q_2,...,q_{n-1}$. $G~0~1$ has the similar meaning.
    \item  $\texttt{Relabel}(\pi,\F')$ constructs $\F$ by relabeling the qubits in $\F'$ with a permutation map $\pi$ over $(\Z_n,+)$. We only search a set of possible permutation $\pi$. $\sigma_m$ is the permutation over $(\Z_n,+)$ that $\forall a\in \Z_n,\sigma_m(a) = a+m$.
    
    For example, let $\pi:(0\quad n-1)$ and $\G:=\texttt{H 0}$. Then \texttt{Relabel}($\pi$, $\G$) is a unitary function that apply Hadamard gate on qubit $q_{n-1}$. The database contains a set of known one- and two-qubit unitary gates. Once we successfully synthesize a program we will also insert it into the database. For an $n$-length bit-vector $x$, we use \texttt{map}$(\pi,x)$ to relabel the bits in $x$ with permutation $\pi$. For example, $\map{\pi}{x}= x_{n-1}x_1x_2...x_0$.
    \item $\F_1;\F_2$ is a unitary function $\lambda n. \F_2(n)\F_1(n)$ where $\F_2(n)\F_1(n)$ means the unitary multiplication.
    % \item $\texttt{Ext}(\gamma(n), \F')$ is a unitary function
    % \begin{align*}
    %     \lambda n. \begin{cases}
    %     I_n, \gamma(n) \le 0\\
    %     \F'(\gamma(n)) \otimes I_{n-\gamma(n)}, \gamma(n)>0\\
    %     \end{cases}
    % \end{align*}
    % where $I_n$ is $2^n\times 2^n$ identity unitary.
    \item $\texttt{Fix}_k(\gamma(n),\F_1,\F_2,...,\F_{k},\F_l,\F_r)$ construct a meta program of the form:
    \begin{coq}
Fixpoint $\F$ n :=
    match n with
    | 1 => $\F_1(1)$
    | ...
    | k => $\F_{k}(k)$
    | _ => $\F_l(n);\F(\gamma(n))_{cast};\F_r(n)$
    end.
\end{coq}
where $\F(\gamma(n))_{cast}$ is a unitary that extend the $2^{\gamma(n)}\times 2^{\gamma(n)}$ unitary $\F(\gamma(n))$ to a $2^n\times 2^n$ unitary by composing a $2^{n-\gamma(n)}\times 2^{n-\gamma(n)}$ identity unitary on qubits $q_{\gamma(n)},q_{\gamma(n)+1},...,q_{n-1}$\par
\item $\F::=O_f$ means an quantum oracle based on a classical function $f$. It is only used in the Oracle synthesis problem.
\end{itemize}
\section{Syntax Rule}
We know that each unitary function can be represented by corresponding $\alpha$ under some precondition $h$. The program constructed by our syntax is also a unitary function. When the unitary function generated by a program $\F$ has the same semantic with a unitary function that can be represented by extended path-sums $\alpha$ under precondition $h$, we say
\begin{align}
    \interpret{h}{\F}{\alpha}
\end{align}
The synthesis goal is: given a target $\alpha_{spec}$ and the precondition $h$, construct a program $\F$ that
\begin{align}
    \interpret{h}{\F}{\alpha_{spec}}
\end{align}
When $\F$ is constructed by $G~0$ and $G~0~1$ for some known gate $G$, we suppose already know that $\interpret{h}{\F}{\alpha_G}$. Given arbitrary two path-sums $\alpha, \alpha'$ and function $\gamma_n$, we define
\begin{align}
    \texttt{seq}(\alpha,\alpha') &= \lnxy  \sum_{z\in \{0,1\}^{n}} \alpha(n,x,z)\alpha'(n,z,y)\\
    \texttt{extend}(\gamma(n), \alpha)&=\lnxy \delta(x[n:\gamma(n)+1],y[n:\gamma(n)+1])\nonumber\\
    &*\alpha(\gamma(n),x[\gamma(n):1],y[\gamma(n):1])
\end{align}
If $\alpha, \alpha'$ is equivalent under some precondition $h$ which is checked by SMT solver(discussed in Sec~\ref{sec:express}), we say
\begin{align*}
    \ufeq{h}{\alpha}{\alpha'}
\end{align*}
For the unitary function constructed by our syntax, we have the rules:
\begin{figure*}[h]
\begin{minipage}[m]{0.9\textwidth}
\centering
\begin{gather*}
\infer[\text{(Weaken)}]{\interpret{h'}{\F}{\alpha}}{\begin{array}{c}
     \interpret{h}{\F}{\alpha}  \\
     \forall n~x~y, h(n,x,y)\rightarrow h'(n,x,y)
\end{array}}\\\\
\infer[\text{(Relabel)}]{\interpret{h}{\texttt{Relabel}(\pi,\F')}{\alpha}}{
\begin{array}{c}
    \interpret{h'}{\F'}{\alpha'}\\
    h=\lnxy h'(n,\map{\pi}{x})\\
     \ufeq{h}{\alpha}{\lnxy \alpha'(n, \map{\pi}{x},\map{\pi}{y})}  \\
\end{array}
}\\\\
        \infer[\text{(Sequence)}]{
    \interpret{h}{\F_1;\F_2}{\alpha}
    }{
    \begin{array}{c}
        \interpret{h_1}{\F_1}{\alpha_1}\quad \interpret{h_2}{\F_2}{\alpha_2}   \\
         h =\lnxy\ h_1(n,x) \land (h_1(n,x) \rightarrow \forall y\in \{0,1\}^{n}, h_2(n,y)\rightarrow \alpha_1(n,x,y)\neq 0)\\
         \ufeq{h}{\alpha}{\texttt{seq}(\alpha_1,\alpha_2)}
    \end{array}
    } \nonumber\\\\
    % \infer[\text{(Extend)}]{\interpret{h}{\texttt{Ext}(\gamma(n), \F')}{\texttt{extend}(\gamma(n), \alpha')}}{
    % \begin{array}{cc}
    %   \interpret{h'}{\F'}{\alpha'},\quad \forall n>0, x\in\{0,1\}^{n}, h'(n,x)\rightarrow h'(\gamma(n),x[\gamma(n):1])  \\
    %     h = \lnx h'(n,x)\land \gamma(n)>0  \\
    % \end{array}
    % }\\\\
    \infer[\text{(Fixpoint)}]{\interpret{h}{\texttt{Fix}_k(\gamma(n),\F_0,\F_1,...,\F_{k-1},\F_l,\F_r)}{\alpha}}{
    \begin{array}{c}
         \forall i:0\le i<k, \interpret{h_i}{\F_i}{\alpha_i}, \ufeq{h_i}{\alpha_i}{\alpha}\\
         \text{where }h_i=\lnxy h(n,x,y) \land n==i  \\
         \interpret{h}{\F_l}{\alpha_l}\quad \interpret{\lnx\textbf{True}}{\F_r}{\alpha_r}\\
         \ufeq{h}{\alpha}{\texttt{seq}(\texttt{seq}(\alpha_l, \texttt{extend}(\gamma(n),\alpha)), \alpha_r)} \\
    \end{array}
    }
\end{gather*}
\end{minipage}
\caption{Syntax Rule}
\end{figure*}


==> title.tex <==
%% Title information
       %% 

% \author{First1 Last1}
% \authornote{with author1 note}          %% \authornote is optional;
%                                         %% can be repeated if necessary
% \orcid{nnnn-nnnn-nnnn-nnnn}             %% \orcid is optional
% \affiliation{
%   \position{Position1}
%   \department{Department1}              %% \department is recommended
%   \institution{Institution1}            %% \institution is required
%   \streetaddress{Street1 Address1}
%   \city{City1}
%   \state{State1}
%   \postcode{Post-Code1}
%   \country{Country1}                    %% \country is recommended
% }
% \email{first1.last1@inst1.edu}          %% \email is recommended

% %% Author with two affiliations and emails.
% \author{First2 Last2}
% \authornote{with author2 note}          %% \authornote is optional;
%                                         %% can be repeated if necessary
% \orcid{nnnn-nnnn-nnnn-nnnn}             %% \orcid is optional
% \affiliation{
%   \position{Position2a}
%   \department{Department2a}             %% \department is recommended
%   \institution{Institution2a}           %% \institution is required
%   \streetaddress{Street2a Address2a}
%   \city{City2a}
%   \state{State2a}
%   \postcode{Post-Code2a}
%   \country{Country2a}                   %% \country is recommended
% }
% \email{first2.last2@inst2a.com}         %% \email is recommended
% \affiliation{
%   \position{Position2b}
%   \department{Department2b}             %% \department is recommended
%   \institution{Institution2b}           %% \institution is required
%   \streetaddress{Street3b Address2b}
%   \city{City2b}
%   \state{State2b}
%   \postcode{Post-Code2b}
%   \country{Country2b}                   %% \country is recommended
% }
% \email{first2.last2@inst2b.org}         %% \email is recommended
